Forced Migration and Information-Seeking Behavior on Wikipedia: Insights from the Ukrainian Refugee Crisis

Gathering information about where to migrate is an important part of the migration process, especially during forced migration, when people must make rapid decisions under uncertainty. This study examines how forced migration relates to online information-seeking on Wikipedia. Focusing on the 2022 Russian invasion of Ukraine, we analyze how the resulting refugee crisis, which led to over six million Ukrainians fleeing across Europe, shaped views of Wikipedia articles about European cities. We compare changes in views of Ukrainian-language Wikipedia articles, used as a proxy for information-seeking by Ukrainians, with those in four other language editions. Our findings show that views of Ukrainian-language articles about European cities correlate more strongly with the number of Ukrainian refugees applying for temporary protection in European countries than views in other languages. Because Poland and Germany became the main destinations for refugees, we examine these countries more closely and find that applications for temporary protection in Polish and German cities are also more strongly correlated with views of their Ukrainian-language Wikipedia articles. We further analyze the timing between refugee flows to Poland and online information-seeking. Refugee border crossings occurred before increases in Ukrainian-language views of Polish city articles, indicating that information-seeking surged after displacement. This reactive pattern contrasts with the pre-departure planning typical of regular labor migration. Moreover, while official protection applications often lagged behind border crossings by weeks, Wikipedia activity rose almost immediately. Overall, Wikipedia usage offers a near real-time indicator of emerging migration patterns during crises.

==> todos.tex <==
ARIMA Wikipedia data 08.2020 - 08.2023

Poisson regression

Fixed effects (monthly) city and country (crossing the border or PESEL numbers ~ Wikipedia month fixed effect)
Wikipedia data and Crossing the border starting from 24.02.2022

Google Trends
